PhysioCHI: Towards Best Practices for Integrating Physiological Signals in HCI

Recently, we saw a trend toward using physiological signals in interactive systems. These signals, offering deep insights into users' internal states and health, herald a new era for HCI. However, as this is an interdisciplinary approach, many challenges arise for HCI researchers, such as merging diverse disciplines, from understanding physiological functions to design expertise. Also, isolated research endeavors limit the scope and reach of findings. This workshop aims to bridge these gaps, fostering cross-disciplinary discussions on usability, open science, and ethics tied to physiological data in HCI. In this workshop, we will discuss best practices for embedding physiological signals in interactive systems. Through collective efforts, we seek to craft a guiding document for best practices in physiological HCI research, ensuring that it remains grounded in shared principles and methodologies as the field advances.

==> OLD.tex <==

There is a growing interest in technical development, academic research, and consumer use of biosensing technology. \textbf{Biosensors} or \textbf{physiological sensors} measure our physiological processes (e.g., heart rate, breathing, skin conductance, brain activity, muscle tension), provide \textbf{biofeedback}, and allow us to display our \textbf{biodata} and perceive internal states of our bodies in new ways. Our \textbf{biosignals} can provide useful insights into the internal states, health, and emotions of ourselves and others \cite{shu2018review}. This can allow us to \emph{connect} and better understand our own bodies, as well as connect and better understand other people. Along with the pervasive "quantified self" movement, there has been a rapid adoption of this biosensing technology in the consumer market. %(e.g. high performance training, health monitoring). 
Most consumer biosensing devices target individual health and self-improvement (e.g., fitness and health trackers and meditation apps). But, there are also growing opportunities of sharing biosignals within a social context and accessing other's physiological data. For example, to understand other's emotions and support a sense of intimacy and connection. Finally, there is emerging research in HCI that explores biodata aggregated through biosensing technologies as a design material  \cite{10.1145/3274338, 10.1145/3313831.3376684} for developing systems that can offer novel somatic experiences or extend the knowledge and appreciation of one's body   \cite{10.1145/3411764.3445628}.   






%%% Specific examples
%For example, biodata can give access to a dimension of our experience that ordinarily remains hidden, providing cues indicative of our internal cognitive and affective states. These cues may, for instance, allow for the recognition and training of our attention levels, enable attunement to others' emotions, communication of affective intimate messages, and fostering empathy. Moreover, biosignals may help us to learn to recognize these cues in the absence of technology, as well as to identify emotional and cognitive states which may otherwise be completely hidden. It particularly has potential to aid people with sensory challenges or social disabilities, such as individuals on the autism spectrum \cite{nam2021research}.
%Biosignals may be used for health monitoring, emotion and stress regulation, attention training, affective communication, appreciation of aesthetic experiences, and improving a feeling of connection. 
%Thus, biosignals may provide important implicit physiological cues obscured not only in face-to-face interactions, but also missing from current telepresence and communication technologies including video conferencing and Virtual Reality (VR). Biosignal sharing in social contexts is particularly relevant with the recent dominance of telecommunication as a result of the COVID-19 pandemic, and the associated shortage of rich social affective cues in many of our daily interactions.  It particularly has potential to aid people with sensory challenges or social disabilities, such as individuals on the autism spectrum \cite{nam2021research}.

%%Interest to a broad and diverse CHI community
With the increasing availability of biosensing technologies, there is an uptake of these tools by the CHI community. Integration of biosignals in HCI is a rapidly evolving field that spans different domains including tangible and embodied interaction, affective computing, VR/AR, interactive art, health and wellbeing HCI, cooperative and social computing, game design, body-centric design, and many other communities. A diverse range of biosignals applications have been explored, including: emotion regulation \cite{jervcic2019practicing}, supporting intimacy in long-distance relationships \cite{liu2021significant}, fostering empathy and compassion among strangers in VR \cite{salminen2019evoking}, augmenting social interactions in social VR entertainment \cite{Lee2022}, productivity and feeling human contact in  workplaces \cite{wikstrom2021heart}, meditation \cite{mladenovic2018divsimo}, inviting reflection in public spaces building "smart cities" \cite{howell2019life}, stimulating social exertion in sports and facilitating bodily insight \cite{walmink2014displaying,Karolus2021}, or measuring attention \cite{kosmyna2019attentivu} to monitor engagement of students in the classroom. 

A recent increase in review papers mapping out sections of the domain of design with biosensors reveals the desire of the community to structure and better understand the dimensions of this emerging design space. %, with its associated challenges and opportunities. 
Moge et al. \cite{moge2022shared} presented at CHI'22 a systematic review on interpersonal biofeedback outlining the use of biosignals in social interaction. The authors noted a growing rate of papers over the last 5 years. Prpa et al. \cite{prpa2020inhaling} presented in CHI'20 an analysis of theoretical frameworks underlying design of breath-responsive systems. Yu et al. \cite{yu2018biofeedback} reviewed biofeedback systems for stress management, identifying several challenges pertaining to interpretation of signals, scalability of systems, and sparse evaluation. Feijt et al. \cite{feijt2021sharing} analyzed systems for biofeedback-sharing, exploring its role in interpersonal communication through a communication and media theory lens. Another recent systematic review focuses on the application of physiological data in Virtual Reality (VR) \cite{halbig2021systematic} arguing for how biodata could improve the quality of the interaction in VR, where ordinarily implicit bodily information remains unseen in often emotionless and lifeless avatars.


In this workshop, we will bring together an interdisciplinary community %of researchers, designers, artists, engineers, and policy-makers 
%% The urge to address open questions
Much more research and discussion is needed pertaining to how we \textit{can} and \textit{should} design interactive systems that respond to our physiological activity. There is a particular need to stimulate cross-disciplinary conversations to synthesize common vocabulary, definitions (e.g., what are biosignals), and strategies to address challenges pertaining to use and interpretation, systems implementation, design, implications, and ethics. In this workshop we will bring together an interdisciplinary community %of researchers, designers, artists, engineers, and policy-makers 
to discuss key topics, identify key challenges spanning different domains, and begin to articulate future directions for addressing these challenges. Despite the increasing prominence of biosensing, there is little governance and established best practices for the use of biosensing technology in daily life outside of medical settings. Yet, careless designs and unregulated use of such personal data has the potential to negatively impact users and society as a whole. For example, imbuing biosignals with rich objective interpretations about other's subjective hidden cognitive and affective states may result in inaccurate judgments and discrimination. Neglecting to provide users with agency over their sharing of biosignals can result in issues of privacy and power inequality. This is not only a question of \emph{ethics} and policy as to where and when biosignals can be shared, but also a \emph{design} question of how we interpret and represent biosignals. %The design of their representation will embed different values and meanings within the system which can fundamentally affect how biosignals are perceived and interpreted. 
It is therefore critical to bring together the community %now 
to share our diverse perspectives, and %from research community, interactive art, industry, and policy-makers, 
to synthesize knowledge emerging from practice in order to identify the emerging challenges and begin to formulate guidance for policy and future design developments. 

We aim to bring together the community of researchers, designers, artists and policy makers to explore the challenges occurring in integrating biosignals in HCI.


\textbf{\red{TOPIC 3---Meaning-Making and UX of biodata:}}

The various applications using biosignals reveal the plurality of effects this technology can have on individuals, and our relationship to our own and others' bodies. These effects can have long-term consequences of reshaping these relationships beyond the moment of the interaction. For instance, using biofeedback can improve one's interoceptive awareness (awareness of your internal processes), and receiving information about others' internal state can improve users' ability to understand and empathize with them, ultimately enhancing mutual understanding. This could be particularly useful when only limited affective cues are shared between users, e.g., when interacting using videoconferencing, or when people lack sensitivity to such cues, e.g., with autism. However, this enhanced access to others' states through biosignals also carries the risk of drawing too much attention towards an externalized representation of biodata and away from the human at the other end. Moreover, trusting too much in the accuracy of biodata could develop a false confidence in knowing others' states, while, in reality, biodata might only provide a very limited insight into what others are experiencing \cite{lazar_chapter_2017}. 

Biodata provides us with insights into the state and process of our bodies. However, interpretation of these signals is often ambiguous \cite{howell2016biosignals}. For example, what does it mean if my heart rate is 10 beats faster than my partner's? Considering a case from affective computing, there is a growing debate arising from the constructionist models of emotions \cite{lindquist2022cultural} on how much could be possible to infer from the physiological data about users' emotions given the lack of universal expressions of emotions. How can we design biofeedback systems to avoid over-interpretation and support reflective meaning-making? There is also a challenge of the synthesis of knowledge across diverse applications of biosensing systems, as different fields come from variant theoretical groundings, which results in divergent meaning-making of biodata, as was outlined for breath-responsive systems\cite{prpa2020inhaling}. The influence of context of use presents another challenge for considering variant meaning-making processes. Naturally, our social relationships have a significant effect on our level of comfort with sharing our intimate biodata, as well as the meaning-making we engage in when seeing a representation of a breathing rate depending on whether it comes from a computer, from ourselves, our loved one, our boss, or a stranger. A heartbeat visualization that may be intimate for close relationships \cite{liu2021significant}, feels like oversharing in a professional relationship \cite{qin_having_2020}, or can represent an abstract human unity when received from a distant stranger \cite{lozano-hemmer2019pulse}. 



\textbf{\red{TOPIC X---Designing with and for representing biosignals:} \abdo{merge with meaning making?}}
When designing bio-responsive systems, designers are faced with a challenge of deciding how to represent the signals that they are collecting. Biosignals can be represented in a broad variety of ways ranging from direct display of raw data, skeuomorphic visualizations in social VR \cite{Lee2022}, heavily processed signals with embedded interpretations, to abstract and artistic forms such as varying the appearance of an avatar in VR~\cite{bernal_emotional_2017}. While raw data can be difficult to interpret \cite{slovak_understanding_2012}, processing biodata and presenting it in the form of discrete affective states often is met with skepticism about its accuracy (e.g. \cite{liu2021significant}). Various streams of biodata can also be represented individually \cite{walmink2014displaying} or as an aggregate of signals from a group, potentially overcoming some privacy concerns \cite{qin_having_2020}. Furthermore, while the biofeedback design landscape is dominated by visual representations \cite{lux2018live}, there are open questions in considering how other sensory modalities can be engaged in various contexts. Having multiple users opens many options in how the signals can be mapped and represented for each individual user, and whether this representation needs to be symmetrical across users. This choice of modality and the design of the display within that modality will also have a considerable effect on how users interpret biosignals and how implicit or invasive it can be within our already consumed attention spans. 


hrough discussion, we will aim to map out the \textbf{key challenges} and \textbf{opportunities} presented by technology. The three 3 rounds of discussion will build towards this outcome: (a) R1: hands-on provocations (exercises) + discussion; (b) R2: breadth roundtables based on topics (see \autoref{wk_topics}); (c) R3: depth roundtables based on application areas. This way R1 exercise will thematically connect to topics in R2, and will prompt participants to reflect on relevant themes and challenges through hands-on first-person experience. R2 will connect participants across disciplines to stimulate cross-pollination of ideas between subdomains and encourage new connections to generate a wide map of observed challenges. And R3 will allow for a more in-depth discussion of specific challenges between participants who already work in a more narrowly defined field. 



\red{TODO}
\begin{itemize}
    \item \textbf{Introduction:} We will set the goals and schedule of the workshop. We will invite all participants to include their self-introductions on the Slack channel in advance. 
    \item \textbf{Warm-up Speed-Dating Activity:} We will ask participants to spend 2 minutes to present each other and describe their research interestes related to the workshop. 
    \item \textbf{R1 - First Round: Hands-on Provocations and Discussions:} To stimulate reflection on opportunities and challenges emerging with the use of biosignals, we will invite participants to engage in a series of exercises set up in stations. Stations will include a basic biofeedback interface and playful prompt cards. The stations will be designed to prime participants for discussion in the following round by provoking questions and observations relevant to discussion topics. For example, one activity would include a visualisation of all participants' heart rates in ranked order, and a task to guess which heart rate belongs to whom. This would prompt participants to think about their level of interoceptive awareness of their own physiology, how they make meaning from seeing their own and others' heart rates represented as a number or a bar chart, and which effects seeing everyone's biosignals may have on a group dynamic. There will be 4 stations of activities for in-person participants, 2 stations for a hybrid interaction across participants, and 4 online stations.  
    \item \textbf{R2 - Second Round: Discussion Based on Workshop Topics}. To ensure a breadth of discussion and cross-pollination across diverse fields of participants we will structure the second round based on large common topics across domains and application areas. This will bring together researchers and practitioners across different domains, who struggle with similar challenges. Groups will be tasked with identifying and expanding on a broad set of challenges fitting within each topic. For each identified challenge participants will be asked to %describe it, explain why it is a challenge, 
    unpack it and provide specific examples of where it is being observed, and %rank 
    position it in relation to other challenges in terms of its criticality and solvability. We will provide the groups with a set of prompt cards with some examples of challenges to start off the discussion and blank cards to fill out. Then groups will engage in affinity diagramming to group the cards together to identify common thematic threads. 
    \item \textbf{R3 - Third Round: Discussion Based on Application Areas}. To provide a space for a deeper of prominent challenges observed in each individual application domain, 
    we will group participants based on the application areas they are working in. Here participants will be tasked to select 2-3 challenges from previous round of discussion and brainstorm approaches for addressing these challenges within a specific application domain.
    \item \textbf{Summarizing Findings}: A representative from each group will report on their findings.
    
    This way collectively we will present a map of common challenges and identify future research directions for integrating biosignals in HCI. We will document these finding by saving the Miro board and Presentations containing affinity diagrams, and taking pictures of the white boards in the conference room. We will use these notes for writing a blog post on Medium.com, and reporting the observation in the ACM Interactions Magazine article.
    %\item \textbf{Social Spaces} at the end after workshop. We will invite virtual participants to move into a virtual social space where they can continue their conversations in an informal setting. The physical participants will be encouraged to go together for dinner or drinks for which we will make a reservation at a local restaurant. Together with the attendees, we will also decide on the preferred Online Social Media space to have an online group/channel for growing the community and staying connected. 
\end{itemize}

\begin{table} 
\begin{tabular}{|l|c|c|}
   \textbf{ Time} & \textbf{Activity} & \textbf{Task Description} \\
    \hline
     9:30-9:45 & Introduction & Arrival and Introduction of the workshop goals and schedule \\
     9:45-10:00 & Attunement & Interoception exercise for connecting with one's body \\
     10:00-11:30 & Hands-on Provocations (R1) & Exercises provoking reflections on workshop topics. Discussion \\
     11:30-11:45 & Coffee Break & \\
     11:45-12:30 & Large Group Discussion & Map out themes emerging from reflection on exercises \\
     \hline
     12:30-13:30 & Lunch & Networking \\
     \hline
     13:30-14:30 & Round tables by topic (R2) & Grouped by discussion topic\\
     14:30-15:00 & Report back & Each group summarizes identified challenges \\
     15:00-15:15 & Coffee break & \\
     15:15-16:15 & Rounds tables (R3)  & Grouped by application areas focused discussion \\
     16:15-17:00 & Large group discussion & Building research agenda and future directions \\
     \hline
     18:00-20:00 & Open Dinner & Networking \\
    \hline 
\end{tabular}
\caption{\red{Workshop Schedule}}
\end{table}
